One-shot Implicit Animatable Avatars with Model-based Priors

Existing neural rendering methods for creating human avatars typically either require dense input signals such as video or multi-view images, or leverage a learned prior from large-scale specific 3D human datasets such that reconstruction can be performed with sparse-view inputs. Most of these methods fail to achieve realistic reconstruction when only a single image is available. To enable the data-efficient creation of realistic animatable 3D humans, we propose ELICIT, a novel method for learning human-specific neural radiance fields from a single image. Inspired by the fact that humans can effortlessly estimate the body geometry and imagine full-body clothing from a single image, we leverage two priors in ELICIT: 3D geometry prior and visual semantic prior. Specifically, ELICIT utilizes the 3D body shape geometry prior from a skinned vertex-based template model (i.e., SMPL) and implements the visual clothing semantic prior with the CLIP-based pretrained models. Both priors are used to jointly guide the optimization for creating plausible content in the invisible areas. Taking advantage of the CLIP models, ELICIT can use text descriptions to generate text-conditioned unseen regions. In order to further improve visual details, we propose a segmentation-based sampling strategy that locally refines different parts of the avatar. Comprehensive evaluations on multiple popular benchmarks, including ZJU-MoCAP, Human3.6M, and DeepFashion, show that ELICIT has outperformed strong baseline methods of avatar creation when only a single image is available. The code is public for research purposes at https://huangyangyi.github.io/ELICIT/.

==> configuration/common_acronyms/specific.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% SOME FREQUENTLY USED ACRONYMS %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





==> configuration/instructions.tex <==
\todo{Before you start:} take a look at the configuration folder. It contains many acronyms and parameters, \eg \smplx, \lookat{highlighting} and more. The config files you will change are 00\_Authors, 00\_Conference for venue and to switch between review/final version, and 04\_Method for your title and method name and website. You can also change text highlighting (02\_Highlight), and add packages (01\_Packages) or parameters (05\_Params). 

Under configuration/common\_acronyms you will find widely used abbreviations and acronyms, for example \rgb, \twod, \twoD, \pseudogt, \etal, and those of existing methods, \eg \smplify, and datasets, \eg \coco.

While writing, it's helpful to color \supmat and \mn - so you don't forget to add what you promised. You can change the colors to black for the final version (configurations/02\_Highlight.tex).

==> figtex/compare-sota.tex <==
\newcommand{\compareSOTACaption}{
Qualitative comparison of novel view synthesis between ELICIT and MonoNHR.
}

\begin{figure}[h]
    \centering
    \includegraphics[width=1.00 \linewidth]{./fig/experiments/compare-mononhr.pdf}
    \captionof{figure}{\compareSOTACaption}
    \label{fig:compare-sota}
    \vspace{-4mm}
\end{figure}




==> tabtex/compare-nvs-h36m.tex <==


\begin{table*}[htbp]
\centering
\begin{tabular}{|c||c|c|c||c|c|c||c|c|c|}
\hline
\multirow{2}{*}{} &
  \multicolumn{3}{c||}{S1$^*$} &
  \multicolumn{3}{c||}{S5$^*$} &
  \multicolumn{3}{c|}{S6$^*$} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{PSNR$\uparrow$} &
  SSIM$\uparrow$ & LPIPS $\downarrow$ &
  \multicolumn{1}{c|}{PSNR$\uparrow$} &
  SSIM$\uparrow$ & LPIPS $\downarrow$ &
  \multicolumn{1}{c|}{PSNR$\uparrow$} &
  SSIM$\uparrow$ & LPIPS $\downarrow$\\ \hline
NB\cite{pengNeuralBodyImplicit2021}   &
  \multicolumn{1}{c|}{} &
    &   &
  \multicolumn{1}{c|}{ } &
    &  &
  \multicolumn{1}{c|}{ } &
    &  \\ \hline
 NHP \cite{kwonNeuralHumanPerformer2021} &
  \multicolumn{1}{c|}{ } &
    &  &
  \multicolumn{1}{c|}{ } &
    &  &
  \multicolumn{1}{c|}{ } &
    &  \\ \hline
Ours & 
  \multicolumn{1}{c|}{ } 
   &  &  &
  \multicolumn{1}{c|}{ } &
    &   &
  \multicolumn{1}{c|}{ } &
     &   \\ \hline\hline
\multirow{2}{*}{} &
  \multicolumn{3}{c||}{S7$^*$} &
  \multicolumn{3}{c||}{S8} &
  \multicolumn{3}{c|}{S9} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{PSNR$\uparrow$} &
  SSIM$\uparrow$ & LPIPS $\downarrow$ &
  \multicolumn{1}{c|}{PSNR$\uparrow$} &
  SSIM$\uparrow$ & LPIPS $\downarrow$ &
  \multicolumn{1}{c|}{PSNR$\uparrow$} &
  SSIM$\uparrow$ & LPIPS $\downarrow$\\ \hline
NB\cite{pengNeuralBodyImplicit2021}   &
  \multicolumn{1}{c|}{ } &
    &   &
  \multicolumn{1}{c|}{ } &
    &  & 
  \multicolumn{1}{c|}{ } &
    &  
   \\ \hline
NHP \cite{kwonNeuralHumanPerformer2021}&
  \multicolumn{1}{c|}{ } &
    &  &
  \multicolumn{1}{c|}{ } &
    &   &
  \multicolumn{1}{c|}{ } &
    &  \\ \hline
Ours &
  \multicolumn{1}{c|}{ } &
    &   &
  \multicolumn{1}{c|}{ } &
     &  &
  \multicolumn{1}{c|}{ } &
    &  
   \\ \hline
\end{tabular}
\caption{\label{table:compare-nvs-h36m}\footnotesize Detailed quantitative results of \textbf{novel view synthesis} on Human3.6M dataset in PSNR, SSIM and lpips. $\uparrow$ higher is better. $\downarrow$ lower is better. $^*$Subjects included in the training set of NHP\cite{kwonNeuralHumanPerformer2021}.\yy{Inprogress.}}
\end{table*}



==> tabtex/compare-nvs-lpips.tex <==


\begin{table*}[htbp]
\centering
\begin{tabular}{|c||c|c|c||c|c|c||c|c|c|}
\hline
\multirow{2}{*}{} &
  \multicolumn{3}{c||}{Subject 313$^*$} &
  \multicolumn{3}{c||}{Subject 377$^*$} &
  \multicolumn{3}{c|}{Subject 386$^*$} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{PSNR$\uparrow$} &
  SSIM$\uparrow$ & LPIPS $\downarrow$ &
  \multicolumn{1}{c|}{PSNR$\uparrow$} &
  SSIM$\uparrow$ & LPIPS $\downarrow$ &
  \multicolumn{1}{c|}{PSNR$\uparrow$} &
  SSIM$\uparrow$ & LPIPS $\downarrow$\\ \hline
NB\cite{pengNeuralBodyImplicit2021}   &
  \multicolumn{1}{c|}{21.07} &
   0.8276& 111.1 &
  \multicolumn{1}{c|}{19.40} &
   0.7838& 136.3 &
  \multicolumn{1}{c|}{21.22} &
   0.7646& 156.1 \\ \hline
 NHP \cite{kwonNeuralHumanPerformer2021} &
  \multicolumn{1}{c|}{24.39} &
   0.8995 & 162.5 &
  \multicolumn{1}{c|}{23.32} &
   0.8824 & 188.8 &
  \multicolumn{1}{c|}{25.36} &
   0.8855 & 218.5 \\ \hline
Ours & 
  \multicolumn{1}{c|}{25.04} 
   & 0.9331 & 65.74 &
  \multicolumn{1}{c|}{23.82} &
   0.9326 &  71.87 &
  \multicolumn{1}{c|}{27.10} &
   0.9345 &  78.99 \\ \hline\hline
\multirow{2}{*}{} &
  \multicolumn{3}{c||}{Subject 392$^*$} &
  \multicolumn{3}{c||}{Subject 393} &
  \multicolumn{3}{c|}{Subject 394} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{PSNR$\uparrow$} &
  SSIM$\uparrow$ & LPIPS $\downarrow$ &
  \multicolumn{1}{c|}{PSNR$\uparrow$} &
  SSIM$\uparrow$ & LPIPS $\downarrow$ &
  \multicolumn{1}{c|}{PSNR$\uparrow$} &
  SSIM$\uparrow$ & LPIPS $\downarrow$\\ \hline
NB\cite{pengNeuralBodyImplicit2021}   &
  \multicolumn{1}{c|}{22.76} &
   0.8400& 114.7 &
  \multicolumn{1}{c|}{19.62} &
   0.7793& 131.8 & 
  \multicolumn{1}{c|}{18.11} &
   0.6797& 173.1 
   \\ \hline
NHP \cite{kwonNeuralHumanPerformer2021}&
  \multicolumn{1}{c|}{24.81} &
   0.8890&  189.2 &
  \multicolumn{1}{c|}{24.26} &
   0.8943&  164.5 &
  \multicolumn{1}{c|}{24.22} &
   0.8715&  191.6 \\ \hline
Ours &
  \multicolumn{1}{c|}{25.68} &
   0.9377 & 70.24 &
  \multicolumn{1}{c|}{24.65} &
    0.9317 & 71.81 &
  \multicolumn{1}{c|}{24.66} &
   0.9200 & 79.83
   \\ \hline
\end{tabular}
\caption{\label{table:compare-nvs} Detailed quantitative results of \textbf{novel view synthesis} on ZJU-MoCap dataset in PSNR, SSIM and lpips. $\uparrow$ higher is better. $\downarrow$ lower is better. $^*$Subjects included in the training set of NHP\cite{kwonNeuralHumanPerformer2021}.\yy{(TODO) reformat the table}}
\end{table*}



==> tabtex/compare-zjumocap.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}

\begin{table*}[htbp]
    \vspace{-4mm}
\centering
\begin{threeparttable}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{c|c|ccccccccc|ccccccccc} 
\multicolumn{1}{l|}{\multirow{3}{*}{Dataset}}                         & \multirow{3}{*}{Subjects} & \multicolumn{9}{c|}{\textbf{Novel View Synthesis}}                                                                                                                                                                 & \multicolumn{9}{c}{\textbf{Novel Pose Synthesis}}                                                                                                                                                                          \\
\multicolumn{1}{l|}{}                                                 &                           & \multicolumn{3}{c}{PSNR$\uparrow$}                              & \multicolumn{3}{c}{SSIM$\uparrow$}                                 & \multicolumn{3}{c|}{LPIPS$\downarrow$}                             & \multicolumn{3}{c}{PSNR$\uparrow$}                                 & \multicolumn{3}{c}{SSIM$\uparrow$}                                   & \multicolumn{3}{c}{LPIPS$\downarrow$}                                 \\
\multicolumn{1}{l|}{}                                                 &                           & NB   & NHP  & {\cellcolor{Gray}}ELICIT        & NB    & NHP   & {\cellcolor{Gray}}ELICIT         & NB    & NHP   & {\cellcolor{Gray}}ELICIT         & NB   & AniNeRF & {\cellcolor{Gray}}ELICIT        & NB    & AniNeRF & {\cellcolor{Gray}}ELICIT         & NB    & AniNeRF & {\cellcolor{Gray}}ELICIT          \\ 
\shline
\multirow{10}{*}{\begin{tabular}[c]{@{}c@{}}ZJU-\\MoCap\end{tabular}} 
& $313$*  & 21.1 & 24.0 & {\cellcolor{Gray}}\textbf{24.7} & 0.828 & 0.896 & {\cellcolor{Gray}}\textbf{0.931} & 0.237 & 0.168 & {\cellcolor{Gray}}\textbf{0.068} & 20.9 & 20.8   & {\cellcolor{Gray}}\textbf{24.5} & 0.800 & 0.816  & {\cellcolor{Gray}}\textbf{0.933} & 0.278 & 0.237  & {\cellcolor{Gray}}\textbf{0.061}  \\
& $315$*  & 17.8 & 19.0 & {\cellcolor{Gray}}\textbf{22.1} & 0.779 & 0.828 & {\cellcolor{Gray}}\textbf{0.925} & 0.255 & 0.222 & {\cellcolor{Gray}}\textbf{0.073} & 18.2 & 18.5   & {\cellcolor{Gray}}\textbf{21.8} & 0.747 & 0.782  & {\cellcolor{Gray}}\textbf{0.921} & 0.309 & 0.297  & {\cellcolor{Gray}}\textbf{0.075}  \\
& $377$*  & 19.4 & 23.1 & {\cellcolor{Gray}}\textbf{23.6} & 0.784 & 0.879 & {\cellcolor{Gray}}\textbf{0.931} & 0.273 & 0.193 & {\cellcolor{Gray}}\textbf{0.074} & 18.2 & 19.5   & {\cellcolor{Gray}}\textbf{24.6} & 0.686 & 0.788  & {\cellcolor{Gray}}\textbf{0.939} & 0.362 & 0.293  & {\cellcolor{Gray}}\textbf{0.063}  \\
& $386$*  & 21.2 & 25.1 & {\cellcolor{Gray}}\textbf{26.9} & 0.886 & 0.882 & {\cellcolor{Gray}}\textbf{0.933} & 0.312 & 0.225 & {\cellcolor{Gray}}\textbf{0.081} & 22.0 & 24.3   & {\cellcolor{Gray}}\textbf{24.5} & 0.745 & 0.824  & {\cellcolor{Gray}}\textbf{0.910} & 0.357 & 0.289  & {\cellcolor{Gray}}\textbf{0.095}  \\
& $387$   & 17.7 & 21.0 & {\cellcolor{Gray}}\textbf{22.9} & 0.760 & 0.865 & {\cellcolor{Gray}}\textbf{0.920} & 0.283 & 0.190 & {\cellcolor{Gray}}\textbf{0.088} & 18.5 & 19.8   & {\cellcolor{Gray}}\textbf{22.7} & 0.743 & 0.813  & {\cellcolor{Gray}}\textbf{0.922} & 0.316 & 0.266  & {\cellcolor{Gray}}\textbf{0.083}  \\
& $390$*  & 19.2 & 23.6 & {\cellcolor{Gray}}\textbf{25.0} & 0.706 & 0.871 & {\cellcolor{Gray}}\textbf{0.924} & 0.357 & 0.208 & {\cellcolor{Gray}}\textbf{0.086} & 20.2 & 20.8   & {\cellcolor{Gray}}\textbf{24.0} & 0.675 & 0.773  & {\cellcolor{Gray}}\textbf{0.921} & 0.377 & 0.298  & {\cellcolor{Gray}}\textbf{0.076}  \\
& $392$*  & 22.8 & 24.7 & {\cellcolor{Gray}}\textbf{25.6} & 0.840 & 0.887 & {\cellcolor{Gray}}\textbf{0.936} & 0.229 & 0.193 & {\cellcolor{Gray}}\textbf{0.072} & 20.9 & 19.3   & {\cellcolor{Gray}}\textbf{24.3} & 0.742 & 0.786  & {\cellcolor{Gray}}\textbf{0.931} & 0.339 & 0.293  & {\cellcolor{Gray}}\textbf{0.070}  \\
& $393$   & 19.6 & 24.0 & {\cellcolor{Gray}}\textbf{24.5} & 0.779 & 0.892 & {\cellcolor{Gray}}\textbf{0.930} & 0.264 & 0.168 & {\cellcolor{Gray}}\textbf{0.074} & 18.8 & 19.6   & {\cellcolor{Gray}}\textbf{23.7} & 0.752 & 0.784  & {\cellcolor{Gray}}\textbf{0.926} & 0.255 & 0.274  & {\cellcolor{Gray}}\textbf{0.072}  \\
& $394$   & 18.1 & 24.1 & {\cellcolor{Gray}}\textbf{24.5} & 0.680 & 0.869 & {\cellcolor{Gray}}\textbf{0.918} & 0.346 & 0.196 & {\cellcolor{Gray}}\textbf{0.082} & 19.4 & 22.8   & {\cellcolor{Gray}}\textbf{24.8} & 0.715 & 0.858  & {\cellcolor{Gray}}\textbf{0.920} & 0.337 & 0.181  & {\cellcolor{Gray}}\textbf{0.073}  \\
& Average & 19.9 & 23.1 & {\cellcolor{Gray}}\textbf{24.4} & 0.795 & 0.875 & {\cellcolor{Gray}}\textbf{0.929} & 0.276 & 0.196 & {\cellcolor{Gray}}\textbf{0.077} & 19.7 & 20.3   & {\cellcolor{Gray}}\textbf{23.8} & 0.736 & 0.796  & {\cellcolor{Gray}}\textbf{0.925} & 0.324 & 0.276  & {\cellcolor{Gray}}\textbf{0.074}  \\ 
\midrule
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Human\\3.6M\end{tabular}}  
& S1*      & 18.3 & \textbf{25.1} & {\cellcolor{Gray}}24.2 & 0.710 & 0.896 & {\cellcolor{Gray}}\textbf{0.920} & 0.328 & 0.121 & {\cellcolor{Gray}}\textbf{0.065} & 21.6 & 21.5   & {\cellcolor{Gray}}\textbf{25.7} & 0.843 & 0.842  & {\cellcolor{Gray}}\textbf{0.933} & 0.224 & 0.212  & {\cellcolor{Gray}}\textbf{0.061}  \\
& S5*      & 19.7 & \textbf{25.1} & {\cellcolor{Gray}}24.0 & 0.785 & 0.895 & {\cellcolor{Gray}}\textbf{0.918} & 0.266 & 0.126 & {\cellcolor{Gray}}\textbf{0.076} & 21.3 & 22.0   & {\cellcolor{Gray}}\textbf{23.5} & 0.828 & 0.821  & {\cellcolor{Gray}}\textbf{0.924} & 0.236 & 0.244  & {\cellcolor{Gray}}\textbf{0.070}  \\
& S6*      & 19.6 & 23.5 & {\cellcolor{Gray}}\textbf{23.7} & 0.777 & 0.839 & {\cellcolor{Gray}}\textbf{0.912} & 0.257 & 0.160 & {\cellcolor{Gray}}\textbf{0.074} & 21.7 & 21.2   & {\cellcolor{Gray}}\textbf{24.8} & 0.820 & 0.812  & {\cellcolor{Gray}}\textbf{0.924} & 0.230 & 0.237  & {\cellcolor{Gray}}\textbf{0.071}  \\
& S7*      & 18.6 & 23.9 & {\cellcolor{Gray}}\textbf{23.9} & 0.751 & 0.856 & {\cellcolor{Gray}}\textbf{0.919} & 0.299 & 0.153 & {\cellcolor{Gray}}\textbf{0.076} & 18.3 & 20.2   & {\cellcolor{Gray}}\textbf{25.3} & 0.771 & 0.783  & {\cellcolor{Gray}}\textbf{0.928} & 0.297 & 0.280  & {\cellcolor{Gray}}\textbf{0.070}  \\
& S8      & 18.2 & 20.5 & {\cellcolor{Gray}}\textbf{22.1} & 0.778 & 0.838 & {\cellcolor{Gray}}\textbf{0.912} & 0.254 & 0.166 & {\cellcolor{Gray}}\textbf{0.081} & 21.2 & 22.0   & {\cellcolor{Gray}}\textbf{25.2} & 0.847 & 0.863  & {\cellcolor{Gray}}\textbf{0.932} & 0.220 & 0.191  & {\cellcolor{Gray}}\textbf{0.063}  \\
& S9      & 20.8 & 23.0 & {\cellcolor{Gray}}\textbf{25.0} & 0.780 & 0.818 & {\cellcolor{Gray}}\textbf{0.910} & 0.261 & 0.192 & {\cellcolor{Gray}}\textbf{0.082} & 22.1 & 22.3   & {\cellcolor{Gray}}\textbf{25.9} & 0.811 & 0.815  & {\cellcolor{Gray}}\textbf{0.925} & 0.250 & 0.236  & {\cellcolor{Gray}}\textbf{0.069}  \\
& S11     & 21.2 & 22.5 & {\cellcolor{Gray}}\textbf{25.5} & 0.783 & 0.822 & {\cellcolor{Gray}}\textbf{0.921} & 0.280 & 0.201 & {\cellcolor{Gray}}\textbf{0.082} & 20.9 & 23.7   & {\cellcolor{Gray}}\textbf{25.7} & 0.809 & 0.858  & {\cellcolor{Gray}}\textbf{0.934} & 0.272 & 0.224  & {\cellcolor{Gray}}\textbf{0.064}  \\
& Average & 19.5 & 23.4 & {\cellcolor{Gray}}\textbf{24.1} & 0.766 & 0.852 & {\cellcolor{Gray}}\textbf{0.916} & 0.278 & 0.160 & {\cellcolor{Gray}}\textbf{0.077} & 21.0 & 21.8   & {\cellcolor{Gray}}\textbf{25.2} & 0.818 & 0.828  & {\cellcolor{Gray}}\textbf{0.928} & 0.247 & 0.232  & {\cellcolor{Gray}}\textbf{0.067}   \\
\end{tabular}
}
\end{threeparttable}
    \vspace{-2mm}
\caption{\footnotesize\label{table:compare-zjumocap} Detailed quantitative results of \textbf{novel pose synthesis} and \textbf{novel pose synthesis} on \textbf{ZJU-MoCap}\cite{pengNeuralBodyImplicit2021} and \textbf{Human 3.6M}\cite{ionescu2013human36m} dataset in PSNR$\uparrow$, SSIM$\uparrow$(higher is better) and LPIPS$\downarrow$(lower is better), our method outperforms in both datasets compared to the per-subject optimization baseline NeuralBody\cite{pengNeuralBodyImplicit2021}(NB) and Animatable NeRF\cite{pengAnimatableImplicitNeural2022, pengAnimatableNeuralRadiance2021a}(AniNeRF), also the generalizable baseline Neural Human Performer(NHP) which is pretrained on part of the subjects.   * Subjects included in training set of NHP. }
\vspace{-6mm}
\end{table*}
